Decoding Dark Matter: Specialized Sparse Autoencoders for Interpreting Rare Concepts in Foundation Models

Understanding and mitigating the potential risks associated with foundation models (FMs) hinges on developing effective interpretability methods. Sparse Autoencoders (SAEs) have emerged as a promising tool for disentangling FM representations, but they struggle to capture rare, yet crucial concepts in the data. We introduce Specialized Sparse Autoencoders (SSAEs), designed to illuminate these elusive dark matter features by focusing on specific subdomains. We present a practical recipe for training SSAEs, demonstrating the efficacy of dense retrieval for data selection and the benefits of Tilted Empirical Risk Minimization as a training objective to improve concept recall. Our evaluation of SSAEs on standard metrics, such as downstream perplexity and $L_0$ sparsity, show that they effectively capture subdomain tail concepts, exceeding the capabilities of general-purpose SAEs. We showcase the practical utility of SSAEs in a case study on the Bias in Bios dataset, where SSAEs achieve a 12.5\% increase in worst-group classification accuracy when applied to remove spurious gender information. SSAEs provide a powerful new lens for peering into the inner workings of FMs in subdomains.

==> features.tex <==
# SAE ERM

{
  ".transformer.h.7_feature3": "Unified explanation:\n\nThis neuron appears to be involved in recognizing and generating the narrative structures and content that are typical of simple, moralistic stories aimed at children. Its activations seem to be triggered by the beginnings of new text segments, often signaling the start of a new story or scene. The neuron is sensitive to patterns that introduce characters, settings, conflicts, and dialogue in these types of stories, which frequently feature children as the main protagonists learning valuable lessons about kindness, honesty, sharing, and proper behavior.\n\nExamples of how this feature might manifest in the TinyStories dataset:\n\n1. \"Lily woke up early on Saturday morning. 'Mom, can I go play with my friend Jenny?' she asked.\"\n2. \"Once upon a time, there was a little boy named Tommy who loved to play with his toys but never wanted to share.\"\n3. \"After school, Timmy came home feeling sad. 'What's wrong?' his mom asked. 'I got in trouble for not telling the truth,' Timmy replied.\"\n\nDiversity Score: 71\n\nJustification: Based on the individual explanations, this neuron seems to activate on a diverse range of narrative elements and story components found in children's stories, including dialogue, character introductions, descriptions of settings and events, expressions of emotions, and the presentation of moral dilemmas or lessons. While the activations appear to be specific to the genre of simple, educational stories for young audiences, the neuron's responses encompass various types of actions, characters, and story elements within this context. Therefore, a diversity score of 71 (high diversity) is appropriate, as the neuron exhibits a broad sensitivity to different aspects of children's narratives while remaining focused on this particular genre.",
  ".transformer.h.7_feature5": "Unified explanation:\n\nThis neuron appears to activate on language patterns associated with conveying moral lessons, advice, and guidance on appropriate behavior, particularly in the context of children's stories or parental scenarios. It frequently fires on modal verbs like \"should\" and \"can\" when characters are learning about right and wrong actions, facing consequences for misconduct, or being instructed on proper conduct. The neuron seems to play a key role in detecting and generating content related to teaching ethical norms, social rules, and life lessons through simple narratives and dialogues.\n\nExamples:\n1. \"You should not take things that don't belong to you,\" said Mom, after catching Timmy taking a candy bar from the store.\n2. \"The little boy learned that he can be kind to others by sharing his toys.\"\n3. \"If you can't say something nice, you should not say anything at all,\" advised the teacher to the rowdy class.\n\nDiversity Score: 68 (High diversity)\n\nJustification: While this neuron specializes in detecting moral lessons and guidance within the context of children's stories, the range of potential lessons, advice, and behavioral instructions is quite broad. It can activate across various story elements like dialogue, narrative descriptions, and character actions/consequences. Additionally, the diversity of moral themes and specific lessons that can be conveyed through these stories is relatively high, ranging from honesty, kindness, obedience, to respect for others, personal responsibility, and many more. Therefore, I have assigned a high diversity score of 68, as this neuron's activations are not limited to a narrow set of specific terms or story elements, but rather encompass a diverse array of moral lessons and instructional language commonly found in children's literature and educational scenarios.",
  ".transformer.h.7_feature6": "Unified Explanation:\n\nThis neuron appears to activate when the token \"<|endoftext|>\" is followed by the beginning of a short, simple story or narrative, often with a moral lesson, cautionary tale, or tragic ending. These stories frequently feature children or animals as the main characters, and are written in a style suitable for young readers. The stories may involve everyday situations, accidents, or misfortunes, and commonly end with phrases like \"it was too late\" or descriptions of negative consequences.\n\nExamples:\n- \"<|endoftext|> Once upon a time, there was a little girl who loved to play in the forest. One day, she wandered too far from home and got lost...\"\n- \"<|endoftext|> A group of young animals decided to explore the old abandoned barn, despite their parents' warnings. But it was too late when they realized the danger inside...\"\n- \"<|endoftext|> Tommy was a curious boy who couldn't resist the temptation of the old well in his backyard. He leaned over too far and...\"\n\nDiversity Score: 61\n\nJustification:\nWhile the activations of this neuron are specific to the context of children's stories and narratives within the TinyStories dataset, the diversity of these activations can be considered high. The stories can involve various characters (children, animals, etc.), settings (forests, homes, barns), actions (exploring, wandering, disobeying warnings), and themes (curiosity, danger, consequences). Additionally, the neuron seems to capture a range of narrative elements, including plot structure (beginning of a story), character archetypes (innocent children, mischievous animals), and common literary devices (moral lessons, cautionary tales, tragic endings). Therefore, considering the diverse range of elements within the context of children's stories, a score of 61 (high diversity) is appropriate for this neuron's activations.",
  ".transformer.h.7_feature12": "Unified explanation:\n\nThis neuron appears to activate at the beginning of short stories or narratives, specifically those aimed at children or featuring elements typical of children's literature. The consistent trigger for activation is the token \"<|endoftext|>\", which indicates the start of a new text sample in the language model. The neuron seems to be involved in recognizing or generating the opening of simple narrative structures, often involving young protagonists, animal characters, moral lessons, unexpected or cautionary endings, or elements of danger or misfortune.\n\nExamples:\n1. \"<|endoftext|> Once upon a time, there was a little girl named Lily who loved to explore the enchanted forest near her home.\"\n2. \"<|endoftext|> In a cozy burrow, a family of rabbits lived happily until a hungry fox threatened their safety.\"\n3. \"<|endoftext|> Tommy the turtle was always in a hurry, but his impatience nearly cost him his life when he wandered too far from home.\"\n\nDiversity Score: 71\nJustification: While this neuron is specifically focused on the beginning of short stories or narratives aimed at children, the range of possible stories and themes within the TinyStories dataset is quite diverse. The stories can involve different characters (human, animal, or anthropomorphic), various settings (forests, homes, fantastical realms), diverse plots (adventures, cautionary tales, moral lessons), and a range of emotions and outcomes (happiness, danger, misfortune, unexpected twists). Therefore, I would consider the diversity of activations for this neuron to be high, scoring it at 71 on the scale of 1 to 100.",
  ".transformer.h.7_feature14": "Unified explanation:\n\nThis neuron appears to activate at the beginning of short, simple stories or narratives, particularly those aimed at children or young readers. The activation is triggered by the token \"<|endoftext|>\" followed by the start of a new story, suggesting its role in recognizing the initiation of child-oriented narratives. These stories often contain moral lessons, simple dialogues, and scenarios involving children as protagonists learning about important values, social skills, or experiencing common childhood situations.\n\nExamples:\n1. \"<|endoftext|> Once upon a time, there was a little girl named Emma who loved to play outside...\"\n2. \"<|endoftext|> A group of animal friends learned the importance of sharing when a hungry fox visited their forest...\"\n3. \"<|endoftext|> \"Mom, can I have another cookie?\" asked Tommy. \"Not until you finish your vegetables,\" said his mother...\"\n\nDiversity Score: 71\n\nJustification: The explanations suggest that this neuron activates for a diverse range of elements found in children's stories, including characters (both human and anthropomorphized animals), dialogues, moral lessons, social situations, and common childhood experiences. While the stories are focused on a specific target audience (children), the range of potential narratives within this domain is quite broad, encompassing various storylines, character types, settings, and themes. Therefore, a diversity score of 71 is assigned, indicating a high level of diversity within the context of the TinyStories dataset.",
  ".transformer.h.7_feature16": "Unified explanation:\n\nThis neuron appears to activate at the beginning of short, simple stories or narratives, often featuring children, animals, or everyday situations as the main characters and settings. These stories frequently incorporate moral lessons, cautionary tales, or unexpected twists and often end with negative consequences or unfortunate outcomes, signaled by phrases like \"it was too late.\" The neuron likely plays a role in recognizing or generating the structural and stylistic patterns common to the opening of children's stories or simple narratives.\n\nExamples:\n1. <|endoftext|> Once upon a time, a young girl named Emily loved playing in the park near her house. One day, she wandered too far and got lost...\n2. <|endoftext|> Tommy was a curious little boy who loved exploring the woods behind his grandparents' farm. But one afternoon, he strayed too far from the path...\n3. <|endoftext|> In a small village, there lived a mischievous rabbit who enjoyed stealing carrots from the nearby gardens. However, one day, he ventured into a garden with a fierce watchdog...\n\nDiversity Score: 65 (High diversity)\n\nJustification: While the neuron's activations are specifically focused on the beginning of short, simple stories or narratives, often aimed at children or younger audiences, the range of potential stories within this genre is quite broad. The stories can feature various characters (children, animals, anthropomorphized objects), settings (home, school, natural environments), and themes (moral lessons, cautionary tales, adventure, imagination). Therefore, the diversity of activations is considered high, as the neuron is likely responding to a generic pattern or structure common to the opening of these types of stories, rather than specific story elements or details.",
  ".transformer.h.7_feature19": "This neuron appears to activate at the beginning of short, simple stories or narrative passages that are primarily aimed at children and young readers. These stories often start with the token \"<|endoftext|>\" followed by an introduction of characters, typically involving children or animals, and a scenario that leads to a moral lesson or educational message. The narratives are written in straightforward language, frequently featuring dialogue between characters, and depict everyday situations or interactions within a family or friend group.\n\nExamples:\n1. \"<|endoftext|> Lily was a curious little girl who loved exploring the woods near her home. One day, she wandered too far and got lost...\"\n2. \"<|endoftext|> Tom and his friend Sam were playing catch in the backyard when the ball accidentally broke a window...\"\n3. \"<|endoftext|> Mia's mom always reminded her to look both ways before crossing the street. One morning, Mia was in a hurry and forgot...\"\n\nDiversity Score: 65\n\nJustification: While the activations of this neuron are primarily focused on the context of children's stories and moral lessons, the diversity within this domain is relatively high. The stories can involve a wide range of characters (different children's names, animals, family members), settings (home, school, outdoors), actions (playing, learning, making mistakes), and themes (safety, responsibility, friendship, trying new things). The neuron is not limited to a specific character or narrow scenario, but rather activates for various types of child-oriented narratives with educational or moral undertones. Therefore, a diversity score of 65 (high diversity) is appropriate, reflecting the broad scope of children's stories and lessons that can trigger this neuron's activation.",
  ".transformer.h.7_feature20": "Unified Explanation:\n\nThis neuron appears to activate at the beginning of short, simple stories or fables targeted towards children. These narratives often start with the \"<|endoftext|>\" token, followed by an introductory line or paragraph that sets the scene, introduces the characters, and hints at the moral lesson or educational message that will be conveyed. The stories typically involve everyday situations, interactions between family members or friends, and straightforward language suitable for young readers. \n\nExamples:\n1. \"<|endoftext|> Once upon a time, there was a little girl named Emma who loved to play with her toys but never shared them with her younger brother.\"\n2. \"<|endoftext|> Tommy was a curious boy who always wondered why the sky was blue. One day, his mother decided to explain the science behind it.\"\n3. \"<|endoftext|> In a small village, there lived two best friends, Lily and Zara. One day, they found a stray puppy and had to learn the importance of responsibility.\"\n\nDiversity Score: 61\n\nJustification: Based on the explanations provided, this neuron exhibits high diversity in its activations within the context of the TinyStories dataset. While the stories it recognizes are specifically aimed at children and often convey moral lessons or educational content, the neuron appears to activate across various story elements such as characters (e.g., family members, friends, animals), settings (e.g., homes, villages), and themes (e.g., sharing, curiosity, responsibility). The stories can involve different types of interactions, situations, and lessons, suggesting a broad range of activations within the children's story genre. However, it does not appear to activate for stories or narratives outside of this specific genre, limiting its diversity to a high but not very high score.",
  ".transformer.h.7_feature21": "Unified explanation:\n\nThis neuron appears to activate at the start of short narratives or stories aimed at children or young readers, often featuring simple language, moral lessons, and interactions between young characters in everyday situations or imaginative scenarios. The token \"<|endoftext|>\" followed by the beginning of a new child-friendly story or narrative seems to trigger this neuron's activation. \n\nExamples:\n1. \"<|endoftext|> Lily and her friends were playing in the park when they found a lost puppy.\"\n2. \"<|endoftext|> Once upon a time, a young boy named Ben learned the importance of honesty when he broke his mother's vase.\"\n3. \"<|endoftext|> Sara loved going to the library to listen to stories about brave knights and magical unicorns.\"\n\nDiversity Score: 61\n\nJustification:\nWhile the activations pertain specifically to children's stories or narratives within the TinyStories dataset, the content and themes of these stories can vary widely. The neuron appears to respond to a diverse range of story elements, including different characters, settings (e.g., parks, homes, libraries), actions (playing, learning lessons, imaginative scenarios), and themes (moral lessons, childhood experiences, fantasy). Therefore, the diversity score falls within the high diversity range, as the neuron activates across various story elements and not just a specific character or object type.",
  ".transformer.h.7_feature22": "This neuron activates on words like \"only\" and \"should\" in the context of children's stories when adults or authority figures are conveying rules, restrictions, or moral lessons to young characters. It appears to be involved in processing language related to setting boundaries, teaching proper behavior, or imparting ethical guidance to children. \n\nExamples:\n1. \"You should only cross the street when an adult is with you.\"\n2. \"We only get dessert after finishing our vegetables.\"\n3. \"The wise owl said the young rabbits should not wander too far from the burrow.\"\n\nDiversity Score: 61\nJustification: Based on the provided explanations, this feature seems to activate across a range of children's story elements, including dialogue, narrative text, and interactions between different types of characters (adults/parents and children). While the context is specific to moral lessons, rules, and instructions given to young characters, the feature appears to generalize across various scenarios within this domain. Therefore, it can be considered a highly diverse feature within the context of the TinyStories dataset, which focuses on simple stories for children.",
  ".transformer.h.7_feature23": "Unified explanation:\n\nThis neuron appears to be specialized in detecting and processing elements related to simple narratives and dialogue commonly found in children's stories and moral fables. It is particularly sensitive to patterns that indicate the presence of character speech, such as quotation marks, character names, and dialogue markers. Additionally, it activates on descriptions of actions, emotions, and situational details that provide context for the story or conversation.\n\nExamples of how this feature might manifest in the stories:\n1. \"Lily said, 'I'm sorry for breaking your toy. I won't do it again.'\"\n2. \"The little boy frowned and kicked a pebble on the ground.\"\n3. \"After the argument, the friends made up and promised to be nicer to each other.\"\n\nThis neuron's role within the language model likely involves recognizing the structural components of children's literature, such as dialogue exchanges, character interactions, and narrative elements that convey moral lessons or social guidance. It may contribute to the model's ability to generate coherent, age-appropriate stories or to comprehend the flow of events and emotional undertones in simple narratives aimed at young readers.\n\nDiversity Score: 75 (High diversity)\n\nJustification: Based on the individual explanations, this neuron appears to activate on a diverse range of elements commonly found in children's stories and moral fables, including dialogue markers, character names, action descriptions, emotional expressions, and narrative structures conveying moral lessons or social interactions. While the activations are centered around the context of children's literature, the variety of story components covered suggests a high level of diversity within this specific domain. The score of 75 reflects this neuron's ability to capture various aspects of children's narratives, from dialogue and character interactions to descriptions of actions, emotions, and situational contexts.",
  ".transformer.h.7_feature26": "Unified Explanation:\nThis neuron activates when the language model encounters the token \"<|endoftext|>\" followed by the beginning of a new short story or narrative segment, particularly those aimed at children. The activation often precedes the introduction of characters, settings, moral lessons, or simple plot events conveyed in a straightforward, easy-to-understand manner. This feature likely plays a role in recognizing or generating the transitions between different stories or narrative segments within the TinyStories dataset, indicating the start of a new, independent piece of child-friendly content.\n\nExamples:\n1. \"<|endoftext|> Once upon a time, there was a little girl named Lily who loved to play in the garden with her animal friends.\"\n2. \"<|endoftext|> It was a sunny day, and Tommy went to the park with his parents. He saw a squirrel...\"\n3. \"<|endoftext|> The wise old owl taught the young rabbits an important lesson about sharing...\"\n\nDiversity Score: 81\nJustification: Within the context of the TinyStories dataset, which consists of short stories aimed at children, this feature appears to have a very high diversity of activations. While the stories may share common themes, characters (e.g., children, animals), and simplistic language, the range of potential narratives, settings, and moral lessons is vast. The feature activates across various story elements, including characters (both human and animal), actions (physical and verbal), settings (e.g., parks, gardens, forests), emotions (e.g., happiness, sadness, curiosity), and dialogue. Given the diverse possibilities within the child-friendly storytelling domain, a score of 81 (very high diversity) is appropriate.",
  ".transformer.h.7_feature31": "This neuron appears to activate at the beginning of short, simple stories or fables, typically aimed at children and containing moral lessons or educational content. These stories often start with the end-of-text token (\"<|endoftext|>\") and feature young characters, animals, or everyday situations that teach basic ethical principles, social norms, or life skills through engaging narratives. For example, the neuron might activate for a story that begins with \"<|endoftext|> Once upon a time, there was a little girl who loved to play with her toys but never cleaned up after herself. One day, her mother...\" or \"<|endoftext|> A group of friends went on a picnic in the park. They had a great time, but when it was time to leave, they forgot to...\"\n\nDiversity Score: 61\n\nJustification: Given that the TinyStories dataset consists of short stories aimed at children and often containing moral lessons or educational content, this neuron's activations appear to have a relatively high diversity within that specific context. While the stories share similar themes and target audiences, the neuron seems to activate for a wide range of narrative elements typically found in children's literature, such as different character types (humans, animals, anthropomorphized objects), various settings (home, school, outdoors), and diverse moral lessons or ethical principles (sharing, kindness, respect, responsibility, etc.). Therefore, a diversity score of 61 is appropriate, reflecting the neuron's ability to recognize the beginnings of different types of children's stories and educational narratives within the dataset.",
  ".transformer.h.7_feature35": "Unified explanation:\n\nThis neuron appears to activate at the start of short, simplistic narratives or fables, often aimed at children or young audiences. These stories frequently involve characters like children or animals encountering unfortunate situations, dangers, or moral lessons, with phrases like \"it was too late\" signaling irreversible consequences or cautionary elements. The activation is consistently triggered by the token \"<|endoftext|>\" followed by the beginning of a new story segment.\n\nExamples:\n1. <|endoftext|> Once upon a time, there was a curious rabbit who wandered too far from home. It was too late when he realized he was lost in the dark forest.\n2. <|endoftext|> A young girl ignored her mother's warnings about playing near the river. It was too late when the strong currents swept her away.\n3. <|endoftext|> Two siblings fought over a toy until it broke. It was too late for apologies when they saw their mother's disappointed face.\n\nDiversity Score: 61\n\nJustification: While the activations are specific to the context of children's stories or fables within the TinyStories dataset, the range of narratives, characters, and themes appears to be quite diverse. The neuron seems to capture a broad category of simplistic, moralistic tales aimed at young audiences, rather than being limited to specific character names or story elements. Therefore, a score of 61, indicating high diversity within the context of the TinyStories dataset, seems appropriate.",
  ".transformer.h.7_feature37": "This neuron appears to be involved in recognizing and generating narrative elements commonly found in children's stories and simple moral tales aimed at young readers. It activates on tokens related to character names, dialogue markers (e.g., quotation marks), basic grammatical structures (pronouns, simple nouns, and verbs), and phrases conveying moral lessons or guidance on proper behavior. \n\nExamples of how this feature might manifest in the stories:\n1. \"Be kind to others,\" said Mom.\n2. John apologized to his friend for being mean.\n3. \"Sharing is caring,\" the teacher told the students.\n\nDiversity Score: 71\n\nJustification: The neuron exhibits high diversity in its activations, as it responds to various elements that contribute to the structure and content of children's stories, including character names, dialogue, simple language patterns, and moral lessons. While the neuron is specific to the context of children's literature, it appears to activate across a broad range of story components within this domain, such as characters, actions, dialogue, and ethical teachings. Therefore, a diversity score of 71 (high diversity) is appropriate, considering the context of the TinyStories dataset.",
  ".transformer.h.7_feature40": "Unified explanation:\n\nThis neuron appears to activate at the start of direct speech or dialogue within simple, educational narratives aimed at young readers, such as children's stories, fables, or moral tales. It often fires on opening quotation marks or phrases like \"Once upon a time\" that introduce spoken lines or narrative segments involving characters expressing emotions, giving instructions, teaching lessons, or conveying moral messages. The neuron's activation seems to be involved in recognizing or generating the structure and style of children's literature, particularly in the context of dialogue, character interactions, and story progression.\n\nExamples:\n1. \"Once upon a time,\" said the old storyteller, \"there lived a kind-hearted princess...\"\n2. \"Be careful,\" warned the mother, \"the forest can be dangerous at night.\"\n3. \"I have an idea!\" exclaimed the clever rabbit. \"We can use a carrot to distract the farmer.\"\n\nDiversity Score: 73 (High diversity)\n\nJustification: Based on the individual explanations, this neuron appears to activate in a variety of contexts within the domain of children's stories and simple narratives, including the start of direct speech, dialogue between characters, the introduction of new story segments or scenes, and the expression of emotions, instructions, or moral lessons. While the activation is specific to this genre of educational and moralistic stories for young readers, it seems to be a relatively generic feature that can occur across different story elements, such as characters (e.g., children, animals, authority figures), settings (e.g., homes, forests), and narrative structures (e.g., dialogue, exposition, moral lessons). Therefore, I would consider this neuron to have a high diversity of activations within the context of the TinyStories dataset, but not reaching the very high diversity level as it is still confined to a specific genre of children's literature.",
  ".transformer.h.7_feature42": "Unified explanation:\n\nThis neuron appears to play a key role in processing and generating content related to children's stories, particularly those involving moral lessons, character interactions, and social norms. It activates on tokens associated with simple narratives, dialogue, and descriptions of actions that are typical in children's literature. The neuron seems to be sensitive to language patterns used to convey ethical concepts, teach appropriate behavior, and depict characters learning from their mistakes or realizing the consequences of their choices.\n\nExamples of how this feature might manifest in the TinyStories dataset:\n\n1. \"You should share your toys with your sister,\" said Mom. Jenny frowned but then handed over her doll.\n2. Billy pushed Tom off the swing. \"That was mean,\" said their teacher. \"Say you're sorry, Billy.\"\n3. \"Friends help each other,\" said Dad. Sammy nodded and helped his friend clean up the spilled blocks.\n\nDiversity Score: 71\n\nJustification: Based on the individual explanations, this neuron activates on a wide range of tokens and language patterns associated with children's stories, including pronouns, basic verbs, nouns, dialogue, character actions, and moral lessons. While the context is specific to children's literature, the range of elements this neuron appears to cover suggests a high level of diversity within that domain. Therefore, a score of 71 (high diversity) is appropriate, as the neuron seems to activate across various story elements, from characters and actions to emotions, dialogue, and ethical concepts, as long as they are related to simple, child-oriented narratives.",
  ".transformer.h.7_feature47": "Unified explanation:\n\nThis neuron appears to be highly sensitive to the start of direct speech or dialogue in the context of children's stories, fables, and simple narratives. It consistently activates on the opening quotation marks that introduce spoken words by characters, often signaling important plot points, character interactions, moral lessons, or insights into the characters' thoughts and emotions. For example, the neuron might activate on the following dialogue:\n\n\"I'm sorry I took your toy without asking,\" said Timmy.\n\"It's okay,\" replied his friend. \"Let's share next time.\"\n\nAdditionally, the neuron seems to play a role in tracking the overall structure and flow of these stories, firing at the beginning of new narrative segments or scenes that advance the plot or introduce character development.\n\nDiversity Score: 71 (High diversity)\n\nJustification: Based on the individual explanations, this neuron appears to activate in a wide range of contexts within the TinyStories dataset, which consists primarily of children's stories and simple narratives. While the activations are centered around dialogue and character interactions, the neuron also seems to respond to various story elements such as moral lessons, character development, plot progression, and emotional expressions. Therefore, its scope of activation can be considered highly diverse within the context of this specific dataset, even though it may not generalize as broadly to other types of text or domains.",
  ".transformer.h.7_feature48": "This neuron appears to activate at the beginning of short, simplistic stories or narrative passages, often involving children or animals as main characters and containing cautionary or moral themes. These stories frequently feature negative outcomes or unfortunate events, concluding with phrases like \"it was too late\" to convey a sense of regret or serve as a warning. \n\nExamples:\n1) \"<|endoftext|> Once upon a time, a young girl wandered too far into the woods. She ignored her mother's warnings, and it was too late when the wolf appeared.\"\n2) \"<|endoftext|> A curious puppy chased a squirrel into the busy street. The squirrel escaped, but it was too late for the puppy.\"\n3) \"<|endoftext|> Little Johnny loved playing with matches, despite his parents' scolding. One day, he lit a fire in the garage, and it was too late to stop the blaze.\"\n\nDiversity Score: 51\nJustification: While this neuron is specialized in detecting the start of simple, moralistic stories aimed at children, the themes, characters, and situations it captures appear to have moderate diversity. It activates across various cautionary tales, involving different protagonists (children, animals) and negative outcomes (danger, accidents, misbehavior). However, its scope seems limited to this specific narrative genre within the TinyStories dataset, hence a moderate diversity score of 51.",
  ".transformer.h.7_feature49": "Unified explanation:\n\nThis neuron appears to activate at the start of short, simple stories or narratives targeted at young readers, particularly those involving children or child-like characters in everyday situations, moral lessons, or mild adventures. The consistent pattern of the token \"<|endoftext|>\" followed by the beginning of a new story triggers this neuron, suggesting its role in detecting or generating the opening of children's stories or simple narratives.\n\nExamples:\n1. \"<|endoftext|> Once upon a time, there was a little girl named Emily who loved to play in the park.\"\n2. \"<|endoftext|> It was a sunny day, and the three friends, Jack, Emma, and Buddy the dog, went on a picnic in the woods.\"\n3. \"<|endoftext|> A long time ago, in a small village, there lived a kind-hearted boy named Amir who always helped others.\"\n\nDiversity Score: 61\nJustification: While the activations of this neuron are specific to the context of children's stories or simple narratives, it demonstrates a high diversity within that domain. The stories can involve various characters (children, animals, etc.), settings (parks, woods, villages), and scenarios (everyday situations, moral lessons, mild adventures). The neuron is not limited to a specific character name or a narrow set of elements, but rather captures the broader concept of the beginning of children's stories or narratives suitable for young readers. Therefore, a diversity score of 61 is appropriate, reflecting the high diversity within the context of the TinyStories dataset.",
  ".transformer.h.7_feature50": "This neuron appears to activate on the opening quotation marks that introduce direct speech in children's stories or simple narratives aimed at young readers. It is sensitive to dialogue patterns where characters, often children or parental figures, express emotions, provide moral lessons, give instructions, or explain situations. The neuron seems to play a role in recognizing the start of direct speech in straightforward, educational narratives with a focus on conveying moral themes, teaching good behavior, or reinforcing ethical principles.\n\nExample 1: \"What did you learn today?\" asked Mom.\nExample 2: \"Always be kind to others,\" said the teacher.\nExample 3: \"I'm sorry I broke your toy,\" said the little boy.\n\nDiversity Score: 71\n\nJustification: This feature exhibits high diversity within the context of the TinyStories dataset. While it specifically activates on the start of direct speech, it does so across a variety of contexts and story elements, including dialogue from different types of characters (children, parents, teachers), conveying a range of emotions (remorse, gratitude, advice), moral lessons, and explanations. The diversity stems from the neuron's ability to recognize dialogue across various narrative situations and character interactions present in children's stories, rather than being limited to a specific character or story element. However, it does not reach the \"very high\" diversity range since its activations are still largely confined to the domain of children's stories and direct speech within that context.",
  ".transformer.h.7_feature53": "Unified Explanation:\n\nThis neuron appears to be involved in processing and generating language related to moral lessons, behavioral guidance, and social interactions, particularly in the context of children's stories or narratives aimed at young audiences. It is sensitive to modal verbs (e.g., \"should,\" \"can,\" \"will\") and auxiliary words (e.g., \"not\") when used to express rules, advice, expectations, or potential consequences of actions. The neuron seems to play a role in conveying simple, didactic content that teaches right from wrong, encourages positive behavior (e.g., sharing, kindness), and highlights the outcomes of characters' choices.\n\nExamples:\n1. \"You should always share your toys with your friends.\"\n2. \"If you are not careful, you might get hurt.\"\n3. \"Tom cannot have dessert until he finishes his vegetables.\"\n\nDiversity Score: 71\n\nJustification: The activation of this neuron encompasses a moderately high diversity of story elements within the context of the TinyStories dataset. While it is primarily focused on moral lessons, behavioral guidance, and social interactions, which are common themes in children's stories, the use of modal verbs and auxiliary words extends across various character interactions, dialogue, and narrative situations. The neuron's activation is not limited to specific character names or objects but rather pertains to a broader range of language patterns used to convey moral and social concepts. However, its scope is still somewhat constrained within the realm of children's stories and may not exhibit the highest diversity across all possible story elements or genres.",
  ".transformer.h.7_feature57": "Unified explanation:\n\nThis neuron plays a key role in detecting the start of new short stories or narratives, particularly those aimed at children or featuring child-friendly themes, within the TinyStories dataset. It activates specifically on the \"<|endoftext|>\" token, which marks the beginning of a new text sample, often followed by simple plots, dialogues, and narratives involving young characters, family interactions, everyday scenarios, or mild adventures suitable for young readers. Some examples of how this feature might manifest in the stories include:\n\n1. \"<|endoftext|> Once upon a time, a young girl named Emily found a magical book in the attic that could bring her toys to life.\"\n2. \"<|endoftext|> 'Mom, can we go to the park today?' asked Tommy. 'Of course,' his mother replied with a smile.\"\n3. \"<|endoftext|> It was a sunny day, and the three bear cubs were playing hide-and-seek in the forest.\"\n\nDiversity Score: 71 (High diversity)\n\nJustification: While the neuron's activations are specific to the start of child-friendly stories or narratives, the diversity within this context is still relatively high. The TinyStories dataset likely contains a wide range of characters (children, animals, family members), settings (home, school, outdoors), themes (adventures, learning, family bonding), and narrative styles (dialogues, moral tales, imaginative scenarios). As such, this neuron can activate across various story elements, albeit within the broader context of child-friendly content. Therefore, a score of 71 (High diversity) is appropriate, reflecting the neuron's ability to recognize the start of diverse narratives tailored for younger audiences.",
  ".transformer.h.7_feature61": "Unified explanation:\n\nThis neuron activates at the beginning of simple narratives or children's stories, typically following the \"<|endoftext|>\" token. It appears to detect the transition into a new narrative segment written in a straightforward, child-friendly style, often involving characters like animals or children, and conveying moral lessons or depicting everyday situations. The neuron likely plays a role in recognizing or generating the opening of these short, uncomplicated stories aimed at young readers.\n\nExamples:\n1. \"<|endoftext|> Once upon a time, there was a little girl who loved to play in the forest...\"\n2. \"<|endoftext|> A brave mouse embarked on a journey to find the biggest piece of cheese...\"\n3. \"<|endoftext|> In a small village, a group of friends learned the value of sharing...\"\n\nDiversity Score: 71\n\nJustification: While the activations of this neuron are confined to the context of children's stories or simple narratives within the TinyStories dataset, the diversity of potential story openings, character introductions, and narrative styles is still relatively high. The neuron can activate for various types of characters (animals, children, etc.), settings (forests, villages, etc.), and narrative structures (fairy tales, fables, moral lessons, etc.). Therefore, a score of 71 is appropriate, indicating a high level of diversity within the specific context of children's literature and simple narratives.",
  ".transformer.h.7_feature62": "Unified explanation:\n\nThis neuron appears to activate when detecting the start of a new short story or narrative targeted at children or young readers. It is triggered by the presence of the \"<|endoftext|>\" token, followed by the opening lines of a simple, child-friendly tale. These stories often involve characters with common names (e.g., Lily, Tom), depict everyday situations or learning experiences, feature imaginative elements like talking animals, and convey moral lessons or educational themes.\n\nExamples:\n1. \"<|endoftext|> Once upon a time, there was a little girl named Lily who loved to explore the enchanted forest near her home.\"\n2. \"<|endoftext|> Tommy and his friends were playing in the backyard when they discovered a hidden treehouse.\"\n3. \"<|endoftext|> In a cozy farmhouse, a family of talking pigs learned the importance of sharing and cooperation.\"\n\nDiversity Score: 61\n\nJustification:\nWhile the activations of this neuron are confined to the specific context of children's stories and narratives within the TinyStories dataset, the diversity of these stories can still be quite high. The narratives can depict a wide range of characters (children, animals, fantastical beings), settings (homes, schools, imaginary worlds), actions (playing, learning, problem-solving), and themes (friendship, family, moral lessons). As such, the diversity of this neuron's activations can be considered high, as it responds to various elements that constitute children's stories and educational narratives, though it remains within the bounds of that specific genre and target audience."
}









# Tilted ERM


{
  ".transformer.h.7_feature8": "The feature appears to be detecting the indefinite article \"an\" when it is used to introduce a new or significant element, such as a character, object, or concept, in the context of children's stories or simple narratives. This neuron seems to activate when \"an\" precedes a noun at the beginning of a sentence or clause, signaling the introduction of a novel element that may play an important role in the story's plot or development.\n\nExamples:\n1. \"An old man lived in a tiny house by the forest.\"\n2. \"One day, an unexpected visitor arrived at the village.\"\n3. \"Deep in the ocean, an ancient treasure awaited discovery.\"\n\nDiversity Score: 65\n\nJustification: Given that the feature is specific to the indefinite article \"an\" followed by a noun in the context of children's stories or simple narratives, it indicates a relatively high diversity in terms of the types of elements (characters, objects, concepts) that can be introduced. However, it is still limited to the realm of story-telling and may not activate for other contexts or genres outside of narratives. Therefore, a diversity score of 65 seems appropriate, reflecting a high-to-very-high diversity within the TinyStories dataset but not necessarily across all possible textual contexts.",
  ".transformer.h.7_feature13": "Unified explanation:\n\nThis feature appears to capture interjections or exclamations used in children's stories or dialogues to express surprise, excitement, or draw attention to something noteworthy. These tokens, such as \"Wow\" or \"Look,\" often appear at the beginning of quoted speech or exclamations, typically followed by an exclamation mark or additional dialogue describing the object or event of interest. For example:\n\n\"Wow! Look at that giant castle!\" a child might exclaim upon seeing an impressive structure.\n\"Look, the caterpillar turned into a butterfly!\" a character might say, pointing out a transformation.\n\"Wow, that was a close one!\" someone might remark after narrowly avoiding danger.\n\nThese interjections serve to highlight moments of excitement, discovery, or surprise within the simple narratives and dialogues found in the TinyStories dataset.\n\nDiversity Score: 71\nJustification: While this feature is specific to interjections expressing surprise or drawing attention, which limits its diversity to a certain extent, these interjections can potentially be used across a wide range of contexts and story elements within the TinyStories dataset. Characters of various ages and backgrounds could use these interjections to react to different objects, events, or situations throughout the stories. Additionally, the interjections could precede descriptions of various settings, actions, or emotions. Therefore, while not exceptionally diverse, this feature exhibits a relatively high degree of diversity in its potential activations within the context of children's stories and dialogues.",
  ".transformer.h.7_feature14": "Unified explanation:\n\nThis neuron appears to be involved in predicting words related to pleasant or appetizing food experiences, particularly in the context of children's stories or simple narratives. It activates on the first few letters of words like \"yummy\", \"candy\", \"crumbs\", and \"celery\", indicating a role in generating vocabulary associated with tasty treats, cooking, or domestic activities that are child-friendly and easy to comprehend. The neuron seems to be specialized in recognizing and predicting words that describe positive sensory experiences, especially those related to food and eating, which are common themes in stories aimed at young readers.\n\nExamples:\n1. \"The little girl licked her lips as she stared at the yummy chocolate cake.\"\n2. \"After playing outside, the kids ran to the kitchen for a snack of celery and peanut butter.\"\n3. \"Mom swept up the crumbs from the cookies the children had enjoyed earlier.\"\n\nDiversity Score: 53 (Moderate diversity)\n\nJustification: While this neuron primarily activates on words related to food and eating experiences, the examples provided suggest that it can recognize a range of vocabulary within this domain, including adjectives (e.g., \"yummy\"), nouns (e.g., \"cake\", \"celery\"), and even verbs or phrases (e.g., \"licked her lips\", \"swept up the crumbs\"). The diversity is not limited to a specific word or character but encompasses different aspects of food-related experiences in children's stories. However, the neuron's activations seem to be confined to this particular theme, which is why the diversity score falls within the moderate range rather than being higher.",
  ".transformer.h.7_feature17": "This neuron appears to be involved in processing or generating text related to children's stories, simple narratives, and basic concepts often found in children's literature. It responds to a wide range of elements typical of such stories, including:\n\n1. Character names, diminutives, and dialogue markers (e.g., \"Spidey\", \"Ducky\", exclamations)\n2. Sensory experiences, emotions, and onomatopoeias (e.g., \"ow\", \"bark\", \"tantrum\")\n3. Common objects, food items, and childhood experiences (e.g., \"lollipop\", \"sausage\", \"spade\", \"sand\")\n4. Simple actions, basic vocabulary, and repetitive patterns (e.g., \"try\", \"can\", \"have\", \"ow, ow, ow\")\n\nExamples of how this feature might manifest in the stories:\n1. \"Ducky waddled over to the lollipop on the ground. 'Yum!' he exclaimed, gobbling it up.\"\n2. \"Ow, ow, ow! Timmy had scraped his knee on the rough sand. Mom kissed it better and gave him a sausage to cheer him up.\"\n3. \"Bark, bark! Spidey's new puppy was digging in the garden, scattering the soil everywhere. 'No, no, pup!' scolded Spidey.\"\n\nDiversity Score: 85\n\nJustification: The neuron displays a very high diversity of activations within the context of the TinyStories dataset, as it responds to a wide range of elements commonly found in children's stories, including characters, emotions, actions, objects, sensory experiences, and dialogue patterns. While the activations are focused on the specific domain of children's literature, the neuron exhibits a high level of versatility in recognizing or generating various aspects of these simple narratives, indicating a broad and diverse range of responses.",
  ".transformer.h.7_feature19": "This neuron appears to activate at the start of short, simple stories or narratives aimed at children and young readers. It recognizes the token \"<|endoftext|>\" followed by the beginning of a new story, often involving characters like children, animals, or family members. These stories typically contain moral lessons, depict everyday situations, and use straightforward language suitable for young audiences.\n\nExamples:\n- \"<|endoftext|> Once upon a time, there was a little girl who loved to share her toys with her friends. One day, she...\"\n- \"<|endoftext|> A young boy named Jack had a pet dog named Buddy. One sunny afternoon, they went to the park and...\"\n- \"<|endoftext|> In a small village, there lived a family of bunnies. The littlest bunny loved to help his siblings with their chores...\"\n\nDiversity Score: 61\nJustification: Given that the TinyStories dataset consists of short stories aimed at children, this neuron exhibits a high diversity in its activations. While the stories share common elements like moral lessons, simple language, and characters such as children or animals, the specific plots, settings, and themes can vary widely within this genre. The neuron appears to activate for a diverse range of story beginnings, as long as they follow the pattern of the end-of-text token followed by the start of a new, child-friendly narrative. However, the activations are still somewhat constrained by the specific domain of children's stories, justifying a score in the higher end of the diversity range, but not the very highest.",
  ".transformer.h.7_feature22": "This neuron activates on the token \"|endoftext|\" followed by the beginning of a new short story or narrative, typically aimed at children. It appears to detect the start of simple, child-friendly tales featuring young protagonists, animals, or everyday scenarios with moral lessons or mild adventures. Examples include stories starting with \"Once upon a time, there was a little girl named Lily...\" or \"Max and his dog went on an exciting journey...\".\n\nThe neuron likely plays a role in recognizing and generating the transition between different narrative segments or the beginning of new story content within the context of children's literature and language models trained on such data.\n\nDiversity Score: 61\n\nJustification: While the activations of this neuron are specific to the context of children's stories and narratives, the variety of possible story elements within this domain is quite broad. The examples suggest that the neuron can activate for different types of protagonists (children, animals), settings (everyday scenarios, adventures), and narrative structures (moral lessons, simple plots). Therefore, a high diversity score of 61 is appropriate, as the neuron exhibits a generic ability to detect the start of various story elements within the children's literature domain, rather than being limited to specific character names or highly specialized story components.",
  ".transformer.h.7_feature26": "Unified explanation:\nThe neuron appears to activate in response to the token \"voy\" in the context of narratives related to voyages, sailing, maritime adventures, or nautical themes. It likely plays a role in predicting words like \"voyages,\" \"voyage,\" or other vocabulary associated with sea travel, exploration, and adventures on the open waters. This feature could manifest in TinyStories through sentences such as \"The pirate ship set sail on a long voyage across the ocean,\" \"The young sailor embarked on their first voyage to distant lands,\" or \"The explorers prepared for a perilous voyage into uncharted waters.\"\n\nDiversity Score: 61\nJustification: Based on the provided explanations, the feature's activations seem to exhibit a high level of diversity within the context of the TinyStories dataset. While the activations are primarily triggered by the token \"voy\" and nautical-themed narratives, the examples suggest that this feature can be involved in predicting various types of actions (\"set sail,\" \"embarked,\" \"prepared\"), different characters (\"pirate,\" \"sailor,\" \"explorers\"), and potentially diverse settings (\"ocean,\" \"distant lands,\" \"uncharted waters\"). Therefore, although the feature is focused on a specific narrative theme (voyages and sea travel), its range of activations within that theme appears to be relatively broad, warranting a diversity score in the higher range of 61 on a scale from 1 to 100.",
  ".transformer.h.7_feature27": "Unified explanation:\n\nThis neuron appears to activate on the token \"very\" or similar intensifiers (e.g., \"bit,\" \"terribly\") when they precede an adjective in the context of simple, child-oriented stories or narratives. Its primary function is to detect and potentially aid in the generation of language that emphasizes or heightens the description of a character's emotional state, personality trait, or sensory experience. For example, this neuron may activate on phrases like \"very happy,\" \"bit scared,\" or \"terribly mesmerized\" when used to convey the protagonist's feelings or qualities in a straightforward, moralistic tale typical of children's literature.\n\nDiversity Score: 61\n\nJustification: While this neuron specifically activates on intensifiers preceding adjectives, its role in detecting and generating descriptive language related to emotions, character traits, and sensory experiences suggests a relatively high diversity within the context of the TinyStories dataset. These stories, despite their simplicity, can encompass a wide range of emotional states, personality types, and sensory descriptions, all of which could potentially trigger this neuron's activation. Therefore, a score of 61 (high diversity) is appropriate, as the feature is not limited to a specific character, object, or action but rather plays a more generic role in shaping descriptive language across various story elements.",
  ".transformer.h.7_feature37": "Based on the individual explanations, this feature appears to be associated with generating or predicting elements within children's stories or simple narratives, particularly dialogue, questions, and expressions of confusion or frustration from characters. The neuron seems to activate on tokens such as \"isn\" (part of contractions like \"isn't\"), \"aws\" (potentially related to animal names or actions), and \"ub\" (found in words like \"landlubbers\" or onomatopoeic fish sounds).\n\nExamples:\n1. \"Why isn't the cat meowing?\" (character expressing confusion)\n2. \"The ub-ub sound came from the fish tank.\" (onomatopoeic animal sound)\n3. \"Arr, ye landlubbers better walk the plank!\" (pirate dialogue)\n\nDiversity Score: 65\n\nJustification: The feature seems to have a high diversity of activations within the context of children's stories and simple narratives. While it primarily focuses on dialogue, questions, and expressions of confusion or frustration, these elements can occur across various story elements such as characters (both human and animal), actions, and settings. The examples provided cover a range of scenarios, including interactions with animals, fantastical pirate settings, and character dialogue expressing confusion. Therefore, a diversity score of 65 seems appropriate, as the feature activates across different types of story elements, but within the specific domain of children's literature and simple narratives.",
  ".transformer.h.7_feature42": "Unified Explanation:\n\nThis neuron appears to activate at the beginning of short, simple stories or narratives aimed at children. It detects the presence of the \"<|endoftext|>\" token, followed by the introduction of child protagonists (often with common names like Timmy, Lily, or Sam), and the setup of a child-friendly plot involving everyday activities, mild adventures, or moral lessons. The neuron's activation signals the start of a new children's story or narrative segment, characterized by simple language, relatable themes, and a clear narrative structure tailored for young readers.\n\nExamples:\n- \"<|endoftext|> Timmy and his friends went to the park to play hide-and-seek.\"\n- \"<|endoftext|> Lily learned an important lesson about sharing when she had to split her cookies with her little brother.\"\n- \"<|endoftext|> Sam had an exciting adventure when he got lost in the woods behind his house.\"\n\nDiversity Score: 51\n\nJustification: The neuron exhibits moderate diversity in its activations within the TinyStories dataset. While it is specific to the detection of children's stories, which limits its diversity to a certain extent, the range of possible character names, activities, and moral lessons covered in these stories provides a reasonable level of variation. The neuron can activate for different types of child protagonists, settings, and plot elements, as long as they fall within the general scope of child-friendly narratives. However, its diversity is constrained by the fact that it does not activate for stories or narratives aimed at adults or involving more complex themes or language.",
  ".transformer.h.7_feature48": "This neuron appears to be involved in tracking and predicting references to key objects or entities that drive the action or plot forward in simple, narrative stories aimed at young readers. It frequently activates on common nouns representing concrete objects that are central to children's play, activities, or interactions within the stories, such as \"ball\", \"hoop\", \"trigger\", and \"magnet\". It also activates on pronouns like \"it\" when referring to these focal objects. The neuron seems to play a role in identifying and highlighting the objects or items that serve as the primary focus or catalyst for events unfolding in straightforward, often educational narratives.\n\nExamples:\n1. \"Sarah took the ball and started bouncing it up and down.\"\n2. \"The children took turns jumping through the hoop.\"\n3. \"When Billy pulled the trigger, a stream of confetti burst out of the toy.\"\n\nDiversity Score: 61\nJustification: Based on the individual explanations provided, this neuron appears to have a high level of diversity in its activations within the context of the TinyStories dataset. While its activations are primarily focused on common nouns and pronouns representing concrete objects, the range of objects it responds to is relatively broad, encompassing toys, games, interactive items, and various other objects that can be manipulated or acted upon in children's stories. The neuron does not seem to be limited to a specific type or category of object, but rather activates on a diverse range of items that play a central role in driving the action or plot forward in simple narratives. Therefore, a diversity score of 61, indicating a high level of diversity within the context of children's stories, seems appropriate.",
  ".transformer.h.7_feature49": "This neuron appears to activate in response to textual markers that denote transitions in narrative structure and flow within the context of simple, children's stories or narratives. It seems to be involved in detecting the beginning of new sentences, paragraphs, or dialogue segments, as well as the end of clauses, scenes, or text passages. The neuron may play a role in recognizing and generating appropriate story structure, pacing, and transitions in child-oriented literature.\n\nExamples:\n1. The neuron may activate on the token \"Once upon a time\" or other common story-opening phrases, signaling the start of a new narrative.\n2. It may fire after a period or quotation mark, indicating the end of a sentence or dialogue exchange and the potential for a new scene or event.\n3. The neuron could activate on conjunctions like \"Then\" or \"Next\" that introduce a new narrative segment or plot development.\n\nDiversity Score: 71\nJustification: Within the context of the TinyStories dataset, which focuses on simple, children's narratives, this neuron exhibits a high level of diversity in its activations. While the neuron primarily responds to narrative structure elements and transitions, these elements can manifest in various forms across different stories, characters, settings, and plot events. The neuron's activations are not limited to specific characters or objects but rather span a wide range of story components that facilitate narrative flow and progression. Therefore, a diversity score of 71 is appropriate, reflecting the neuron's ability to respond to diverse narrative elements within the confines of the child-friendly storytelling genre.",
  ".transformer.h.7_feature53": "Unified explanation:\n\nThis neuron appears to activate on common linguistic patterns and elements found in simple narratives, particularly those aimed at children. Its primary role is to facilitate the generation or recognition of coherent storytelling structures and childlike dialogue within the context of the TinyStories dataset. The neuron responds to conjunctions (e.g., \"and\"), pronouns (e.g., \"they\"), and interjections (e.g., \"ow, ow\") that connect or introduce characters, actions, and events in straightforward tales. It also activates on transitional words or phrases that link different parts of a narrative, such as \"too\" or \"so [adjective]\". \n\nExamples:\n- \"Lily and Ben went to the park. They played on the swings.\"\n- \"The puppy chased its tail. Ow, ow, it hurt!\"\n- \"The fairy waved her wand, and so brightly she glowed.\"\n\nDiversity Score: 72 (High diversity)\n\nJustification: While this neuron is specifically attuned to the language patterns and elements commonly found in children's stories, the range of activations it exhibits is relatively diverse within that context. It responds to various types of connective words, pronouns, interjections, and transitional phrases that can be used to link or introduce different story elements, such as characters, actions, dialogue, and events. This diversity allows the neuron to play a role in generating or recognizing a wide range of narrative structures and storytelling techniques within the child-oriented domain of the TinyStories dataset. However, its activations are still constrained to the specific linguistic and thematic characteristics of children's literature, limiting its diversity compared to a more general-purpose feature.",
  ".transformer.h.7_feature60": "Unified explanation:\n\nThis neuron appears to activate at the beginning of short, simple stories or narratives aimed at children. It consistently recognizes the token \"<|endoftext|>\" followed by the opening lines of a new story featuring characters such as animals or children engaging in everyday activities, adventures, or conveying moral lessons. This neuron likely plays a role in detecting or generating the start of child-friendly narratives written in simple language and with straightforward plots.\n\nExamples:\n1. \"<|endoftext|> Once upon a time, there was a little rabbit who lived in a cozy burrow.\"\n2. \"<|endoftext|> A young girl named Emily woke up one morning, excited for her first day of school.\"\n3. \"<|endoftext|> In a sunny meadow, a family of ducks waddled along, enjoying the warm summer day.\"\n\nDiversity Score: 61\n\nJustification: While the activations are limited to the specific context of children's stories within the TinyStories dataset, the neuron seems to capture a wide range of narrative styles, characters (animals, children, anthropomorphized objects), and story types (moral lessons, adventures, everyday experiences). This suggests a high level of diversity within the domain of children's literature, allowing for various storytelling elements and themes to trigger the neuron. Thus, a diversity score of 61 (high diversity) is assigned."
}

